The escape transition of a lattice star polymer grafted in a pore

Polymers in confined spaces are compressed and have reduced conformational entropy, and will partially or fully escape from confinement if conditions are suitable. This is in particular the case for a polymer grafted in a pore. The escape of the polymer from the pore may be considered a partial translocation from the pore into bulk solution, and the resulting conformational readjustment of the polymer has characteristics of a thermodynamic phase transition. In this paper a lattice self-avoiding walk model of a star polymer grafted in a pore is examined numerically using the PERM algorithm. We show that the arms of the grafted lattice star escape one at a time as the length of the pore is reduced, consistent with earlier results in the literature. Critical points for the escape transitions are estimated for square and cubic lattice models and we also examine various properties of the model as it undergoes escape transitions.

==> definition-star-in-pore.tex <==
\begin{figure}[h]
    \beginpicture
    \setcoordinatesystem units <1.5pt,1.5pt>
    \setplotarea x from -70 to 200, y from -10 to 100
    
    \color{Black}
    \arrow <10pt> [.2,.67] from -50 40 to -30 40
    \arrow <10pt> [.2,.67] from -50 40 to -50 60
    \put {\Large$x_1$} at -30 33  \put {\Large$x_2$} at -58 60
    
    
    \color{Tan}
    \setplotsymbol ({\scalebox{1.0}{$\bullet$}})
    \plot 117 -13 117 -3 -3 -3 -3 83 117 83 117 90 / 
    \setplotsymbol ({\scalebox{0.25}{$\bullet$}})
    \setdashes <4pt>
    \plot 118 -13 118 93 /
    \setsolid
    
    \color{Black}
    \setplotsymbol ({\scalebox{0.5}{$\bullet$}})
    \plot 0 40 0 50 10 50 20 50 20 60 20 70 30 70 40 70 50 70 60 70 
    60 60 50 60 50 50 60 50 70 50 80 50 80 60 90 60 100 60 100 70 
    90 70 /
    \plot 0 40 10 40 20 40 30 40 40 40 50 40 60 40 70 40 80 40 90 40
    90 50 100 50 110 50 120 50 130 50 140 50 140 60 130 60 130 70
    140 70 150 70 /
    \plot 0 40 0 30 10 30 20 30 30 30 40 30 40 20 50 20 50 10 60 10 
    70 10 80 10 80 20 70 20 70 30 80 30 90 30 90 20 90 10 100 10 
    110 10 /
    
    \color{White}
    \multiput {{\scalebox{1.5}{$\bullet$}}} at
     0 40 0 50 10 50 20 50 20 60 20 70 30 70 40 70 50 70 60 70 
    60 60 50 60 50 50 60 50 70 50 80 50 80 60 90 60 100 60 100 70 
    90 70 /
    \multiput {{\scalebox{1.5}{$\bullet$}}} at
    0 40 10 40 20 40 30 40 40 40 50 40 60 40 70 40 80 40 90 40
    90 50 100 50 110 50 120 50 130 50 140 50 140 60 130 60 130 70
    140 70 150 70 /
    \multiput {{\scalebox{1.5}{$\bullet$}}} at
    0 40 0 30 10 30 20 30 30 30 40 30 40 20 50 20 50 10 60 10 
    70 10 80 10 80 20 70 20 70 30 80 30 90 30 90 20 90 10 100 10 
    110 10 /
    
    \color{Sepia}
    \multiput {{\scalebox{1.0}{$\bullet$}}} at
     0 40 0 50 10 50 20 50 20 60 20 70 30 70 40 70 50 70 60 70 
    60 60 50 60 50 50 60 50 70 50 80 50 80 60 90 60 100 60 100 70 
    90 70 /
    \multiput {{\scalebox{1.0}{$\bullet$}}} at
    0 40 10 40 20 40 30 40 40 40 50 40 60 40 70 40 80 40 90 40
    90 50 100 50 110 50 120 50 130 50 140 50 140 60 130 60 130 70
    140 70 150 70 /
    \multiput {{\scalebox{1.0}{$\bullet$}}} at
    0 40 0 30 10 30 20 30 30 30 40 30 40 20 50 20 50 10 60 10 
    70 10 80 10 80 20 70 20 70 30 80 30 90 30 90 20 90 10 100 10 
    110 10 /
    
    \circulararc 360 degrees from 120 54 center at 120 50 
    
    \color{Sepia}
    \put {\scalebox{3.0}{$\bullet$}} at 0 40 
    
    \color{Red}
    \setplotsymbol ({\scalebox{0.25}{$\bullet$}})
    \arrow <10pt> [.2,.67] from 0 5 to 110 5
    \arrow <10pt> [.2,.67] from 0 75 to 90 75
    \arrow <10pt> [.2,.67] from 0 95 to 150 95
    
    \arrow <12pt> [.2,.67] from 67 -10 to 115 -10
    \arrow <12pt> [.2,.67] from 53 -10 to 0 -10
    
    \arrow <12pt> [.2,.67] from -12 48 to -12 80 
    \arrow <12pt> [.2,.67] from -12 32 to -12 0 
    \multiput {\scalebox{0.75}{$\bullet$}} at 0 5 0 75 0 95 
    -12 48 -12 32 67 -10 53 -10 /
    
    \color{Black}
    \put {\scalebox{2.0}{$\sigma_1$}} at 98 76
    \put {\scalebox{2.0}{$\sigma_3$}} at 147 86
    \put {\scalebox{2.0}{$\sigma_2$}} at 118 6
    
    \put {\scalebox{2.0}{$w$}} at -15 40 
    \put {\scalebox{1.8}{$L$}} at 60 -10 
    
    
    \color{black}
    \normalcolor
    
    \endpicture
    \caption{A $3$-star in a pore.  The pore has depth $L$ and width
    $w$.  The star is grafted near the middle of the bottom of the pore, and
    its three arms explore conformations inside the pore, and may escape
    into the bulk space by exiting the pore to the right.  The total length $n$ of the star
    is the sum of the lengths $(n_1,n_2,n_3)$ of its arms, and it is (almost) 
    uniform, so that the arms have almost the same lengths:
    $\lfloor n/3\rfloor \leq n_1 \leq n_2\leq n_3 \leq \lceil n/3 \rceil$.
    The \emph{spans} of the arms are denoted by $(\sigma_1,\sigma_2,
    \sigma_3)$, and clearly $0 \leq \sigma_i \leq \lceil n/3 \rceil$.  The
    arms are labelled such that $\sigma_1\leq\sigma_2\leq\sigma_3$.  The 
    total span of the star is the sum $\sigma=\sigma_1+\sigma_2+\sigma_3$.  
    In each arm there may be a first vertex where it escapes the pore.  
    In the figure the third arm escapes the pore, and the first vertex 
    outside the pore is indicated by $O$. The other arms do not escape, but are 
    retracted inside the pore.}
    \label{F2}
    \end{figure}

==> schematic-star-in-pore.tex <==
\begin{figure}
    \beginpicture
\setcoordinatesystem units <1pt,1pt>
\setplotarea x from -70 to 0, y from -10 to 80
\startrotation by 0 -1 about 20 35

\color{Tan}
\setplotsymbol ({\scalebox{1.0}{$\bullet$}})
\plot -13 70 -3 70 -3 -3 43 -3 43 70 53 70 /
\setplotsymbol ({\scalebox{0.2}{$\bullet$}})
\plot -13 60 -3 70 /  \plot -13 50 -3 60 /  \plot -13 40 -3 50 / \plot -13 30 -3 40 /
\plot -13 20 -3 30 /  \plot -13 10 -3 20 / \plot -13  0 -3 10 /  \plot -13 -10 -3 0 /
\plot -3  -13 7 -3 /  \plot  7 -13 17 -3 /  \plot  17 -13 27 -3 /  \plot  27 -13 37 -3 /
\plot  37 -13 54 4 /  \plot  47 -13 54 -6 /  \plot  43 4 53 14 /  \plot  43 14 53 24 /
\plot  43 24 53 34 /  \plot  43 34 53 44 /  \plot  43 44 53 54 /  \plot  43 54 53 64 /
\plot  43 64 48 69 /

\color{black}
\setplotsymbol ({\scalebox{0.5}{$\bullet$}})
\setquadratic
\plot 20 0 30 5 40 20 40 30 30 40 25 50 30 60 35 70 35 80 30 90 30 100
35 110 40 112 /
\plot 20 0 10 5 13 20 15 30 15 40 10 50 10 60 10 70 7 80 0 90 -10 100  /
\setlinear

\color{Sepia}
\put {\scalebox{2.0}{$\bullet$}} at 20 0
\stoprotation


\setcoordinatesystem units <1pt,1pt> point at -200 0 
\setplotarea x from -10 to 70, y from -10 to 80
\startrotation by 0 -1 about 20 35
\color{Tan}
\setplotsymbol ({\scalebox{0.2}{$\bullet$}})
\plot 0 0 0 70 40 70 40 0 0 0 /  \plot 10 0 10 70 /  \plot 20 0 20 70 /
\plot 30 0 30 70 /  \plot 0 10 40 10 /  \plot 0 20 40 20 /  \plot 0 30 40 30 /
\plot 0 40 40 40 /  \plot 0 50 40 50 / \plot 0 60 40 60 /

\setplotarea x from -10 to 70, y from 40 to 80
\setplotsymbol ({\scalebox{1.0}{$\bullet$}})
\plot -13 70 -3 70 -3 -3 43 -3 43 70 53 70 /
\setplotsymbol ({\scalebox{0.2}{$\bullet$}})
\plot -13 60 -3 70 /  \plot -13 50 -3 60 /  \plot -13 40 -3 50 /  \plot -13 30 -3 40 /
\plot -13 20 -3 30 /  \plot -13 10 -3 20 /  \plot -13  0 -3 10 /  \plot -13 -10 -3 0 /
\plot -3  -13 7 -3 /  \plot  7 -13 17 -3 /  \plot  17 -13 27 -3 /  \plot  27 -13 37 -3 /
\plot  37 -13 54 4 /  \plot  47 -13 54 -6 /  \plot  43 4 53 14 /  \plot  43 14 53 24 /
\plot  43 24 53 34 /  \plot  43 34 53 44 /  \plot  43 44 53 54 /  \plot  43 54 53 64 /
\plot  43 64 48 69 /

\color{black}
\setplotsymbol ({\scalebox{0.5}{$\bullet$}})
\plot 20 0 30 0 30 10 40 10 40 20 30 20 30 30 30 40 30 50 20 50
20 60 30 60 40 60 40 70 40 80 50 80 60 80 60 90 50 90 40 90 
30 90 30 80 20 80 10 80 10 90 20 90 20 100 20 110 30 110 40 110
40 100 /
\plot 20 0 10 0 0 0 0 10 10 10 20 10 20 20 20 30 10 30 10 20 
0 20 0 30 0 40 10 40 10 50 0 50 0 60 10 60 10 70 0 70 0 80 -10 80
-10 90 0 90 0 100 10 100 10 110 10 120 0 120 -10 120 -10 110
-10 100 -20 100 /

\color{Sepia}
\put {\scalebox{2.0}{$\bullet$}} at 20 0
\stoprotation

\color{black}\normalcolor
\endpicture
\caption{(Left) A schematic diagram of a $2$-star grafted in a pore.
The two arms of the star explore conformation inside and outside
the pore.  If the pore is deep, then the star is completely retracted 
inside the pore.  If the pore is shallow, or the $2$-star has long arms, 
then one or both arms escape from the pore and explore conformations 
in bulk outside the pore. (Right) A square lattice model of a $2$-star 
grafted in a pore.  The star is grafted in the bottom of the pore at
its central node, and its arms are self-avoiding walks exploring 
conformations inside the pore, and in the bulk lattice to the
right of the pore in this diagram.}
\label{F1}
\end{figure}

